VeRA: Vector-based Random Matrix Adaptation

Low-rank adapation (LoRA) is a popular method that reduces the number of trainable parameters when finetuning large language models, but still faces acute storage challenges when scaling to even larger models or deploying numerous per-user or per-task adapted models. In this work, we present Vector-based Random Matrix Adaptation (VeRA), which significantly reduces the number of trainable parameters compared to LoRA, yet maintains the same performance. It achieves this by using a single pair of low-rank matrices shared across all layers and learning small scaling vectors instead. We demonstrate its effectiveness on the GLUE and E2E benchmarks, image classification tasks, and show its application in instruction-tuning of 7B and 13B language models.

==> tables/reviews_elora.tex <==
\setlength{\tabcolsep}{4pt}
\centering
\footnotesize
\caption{Example answers generated by models finetuned with LoRA and VeRA, with VeRA obtaining a better score. Two and half paragraphs from the VeRA model's output have been omitted.}
\vspace{-0.5em}
\label{tab:reviews_elora}
\begin{tabular}{l | p{6cm} | p{6cm}}
\toprule
& \multicolumn{1}{c}{LoRA} & \multicolumn{1}{c}{VeRA} \\
\midrule 
& \multicolumn{2}{p{12cm}}{Write a symphony concert review, discussing the orchestra's performance and overall audience experience.} \\ 
\midrule
\multirow{1}{*}{\parbox[t]{4mm}{\rotatebox[origin=c]{90}{\textsc{Answer}}}}
& The symphony concert was a truly mesmerizing experience, with the orchestra's performance leaving the audience in awe. The conductor, with his expertise and passion, led the musicians through a series of beautifully composed pieces, each one more captivating than the last. The orchestra's sound was rich and full, with each instrument perfectly balanced and in harmony. The audience was enraptured by the music, and the applause at the end of each piece was thunderous. The concert was a true testament to the power of music and the talent of the musicians. &
The symphony concert held at the Lincoln Center for the Performing Arts on Saturday, March 12th, 2022, was a truly mesmerizing experience. The New York Philharmonic Orchestra, under the direction of Music Director Jaap van Zweden, performed a program of works by Beethoven, Strauss, and Mahler.\newline The concert began with Beethoven's Symphony No. 1, which was a perfect introduction to the evening's program. The orchestra played with precision and energy, capturing the spirit of the piece and transporting the audience to a different time and place. [...]
\\
\midrule
\multirow{1}{*}{\parbox[t]{4mm}{\rotatebox[origin=c]{90}{\textsc{Review}}}}
& Assistant 1 provided a general review of a symphony concert, which was relevant and accurate. However, it lacked specific details such as the location of the concert, the date, the orchestra's name, the conductor's name, and the pieces performed. This lack of detail made the review less helpful and engaging. & Assistant 2 provided a detailed and engaging review of a specific symphony concert. It mentioned the location, date, orchestra's name, conductor's name, and the pieces performed. It also described the audience's reaction to each piece, which added depth to the review. This level of detail made the review more helpful, relevant, accurate, and engaging. \\
\midrule
\parbox[t]{4mm}{\rotatebox[origin=c]{90}{\textsc{Score}}}
& \multicolumn{1}{c}{7} & \multicolumn{1}{c}{\textbf{9}} \\
\bottomrule
\end{tabular}

==> tables/reviews_lora.tex <==
\setlength{\tabcolsep}{4pt}
\centering
\footnotesize
\vspace{-0.5em}
\caption{Example answers generated by models finetuned with LoRA and VeRA, with LoRA obtaining a better score. Parts of answers are omitted due to their length.}
\label{tab:reviews_lora}
\begin{tabular}{l | p{6cm} | p{6cm}}
\toprule
& \multicolumn{1}{c}{LoRA} & \multicolumn{1}{c}{VeRA} \\
\midrule 
& \multicolumn{2}{p{12cm}}{What if Isaac Newton had focused on biology instead of physics?} \\ 
\midrule
\multirow{1}{*}{\parbox[t]{4mm}{\rotatebox[origin=c]{90}{\textsc{Answer}}}}
&
Isaac Newton was a brilliant scientist who made significant contributions to both physics and biology. While he is best known for his work in physics, he also made important discoveries in biology, including the discovery of the laws of motion and the theory of gravity.

[...]
&
If Isaac Newton had focused on biology instead of physics, he may have made significant contributions to the field of biology. Newton was a brilliant scientist and his work in physics revolutionized the field. However, he also had a keen interest in biology and made several observations and insights about the natural world. [...]
\\
\midrule
\multirow{1}{*}{\parbox[t]{4mm}{\rotatebox[origin=c]{90}{\textsc{Review}}}}
& 
Assistant 1's response is somewhat helpful and relevant, but it contains a major inaccuracy. The assistant claims that Isaac Newton made significant contributions to biology, including the discovery of the laws of motion and the theory of gravity. However, these are actually contributions to physics, not biology. The assistant also speculates on what Newton might have studied if he had focused on biology, but these are purely hypothetical and not based on any historical evidence. The assistant's response is detailed and well-structured, but the inaccuracy undermines its overall quality.
& 
Assistant 2's response is less helpful and relevant, and it contains a major inaccuracy. The assistant claims that Isaac Newton was the first to describe the process of photosynthesis. This is incorrect; the process of photosynthesis was not understood until the 19th century, long after Newton's time. The assistant also makes some general observations about Newton's interest in the natural world, but these are not specific to biology and do not provide a clear answer to the user's question. The assistant's response is less detailed and less well-structured than Assistant 1's response, and the inaccuracy further reduces its quality.
\\
\midrule
\parbox[t]{4mm}{\rotatebox[origin=c]{90}{\textsc{Score}}}
& \multicolumn{1}{c}{\textbf{4}} & \multicolumn{1}{c}{2} \\
\bottomrule
\end{tabular}
